Sketching Datasets for Large-Scale Learning (long version)

This article considers "compressive learning," an approach to large-scale machine learning where datasets are massively compressed before learning (e.g., clustering, classification, or regression) is performed. In particular, a "sketch" is first constructed by computing carefully chosen nonlinear random features (e.g., random Fourier features) and averaging them over the whole dataset. Parameters are then learned from the sketch, without access to the original dataset. This article surveys the current state-of-the-art in compressive learning, including the main concepts and algorithms, their connections with established signal-processing methods, existing theoretical guarantees -- on both information preservation and privacy preservation, and important open problems.

==> tikzlibrarymatrices.code.tex <==
% Copyright (c) Antoine Chatalic, 2017-2018.
% MIT License

\newcommand\randomcolor[2]{
	\pgfmathparse{rnd}
	\pgfmathsetmacro\tmpcolorr{\pgfmathresult}
	\pgfmathparse{rnd}
	\pgfmathsetmacro\tmpcolorg{\pgfmathresult}
	\pgfmathparse{rnd}
	\pgfmathsetmacro\tmpcolorb{\pgfmathresult}
	\definecolor{tmpcol}{rgb}{\tmpcolorr,\tmpcolorg,\tmpcolorb}
	\colorlet{#1}{tmpcol!#2!white}
}
\newcommand\randombinary[1]{
	\pgfmathparse{rnd}
	\pgfmathsetmacro\floatrandom{\pgfmathresult}
    \ifthenelse{\lengthtest{\floatrandom pt > 0.5pt}}{
		\colorlet{#1}{\binaryfirstcolor}
    }{
		\colorlet{#1}{\binarysecondcolor}
	}
}
\newcommand\mixedcolor[4]{
	\pgfmathrandom{#3,#4}
	\pgfmathsetmacro\tmpmixing{\pgfmathresult}
	\colorlet{#1}{#2!\tmpmixing!white}
}
\newcommand\pickcolor[5]{
	%\ifrandomcolorsv
	\ifthenelse{\equal{\randomcolorsv}{false}}{
		\colorlet{#1}{#2}
		\ifnoisycolorsv
			\mixedcolor{#1}{#2}{#3}{#4}
		\else
			\colorlet{#1}{#2}
		\fi
	}{
		\ifthenelse{\equal{\randomcolorsv}{binary}}{
			\randombinary{#1}
		}{
			\randomcolor{#1}{#5}
		}
	}
	%\else
	%\fi
}

%\makeatletter
\DeclareRobustCommand{\rvdots}{%
  \vbox{
    \baselineskip4\p@\lineskiplimit\z@
    \kern-\p@
    \hbox{.}\hbox{.}\hbox{.}
}}
%\makeatother
\pgfdeclarepatternformonly{swneStripes}{\pgfpoint{0cm}{0cm}}{\pgfpoint{1cm}{1cm}}{\pgfpoint{1cm}{1cm}}{
	\foreach \i in {0.1, 0.3,...,0.9}{
		\pgfpathmoveto{\pgfpoint{\i cm}{0cm}}
		\pgfpathlineto{\pgfpoint{1cm}{1cm - \i cm}}
		\pgfpathlineto{\pgfpoint{1cm}{1cm - \i cm - 0.1cm}}
		\pgfpathlineto{\pgfpoint{\i cm + 0.1cm}{0cm}}
		\pgfpathclose%
		\pgfusepath{fill}
		\pgfpathmoveto{\pgfpoint{0cm}{\i cm}}
		\pgfpathlineto{\pgfpoint{1cm - \i cm}{1cm}}
		\pgfpathlineto{\pgfpoint{1cm - \i cm + 0.1cm}{1cm}}
		\pgfpathlineto{\pgfpoint{0cm}{\i cm - 0.1cm}}
		\pgfpathclose%
		\pgfusepath{fill}
	}
}

\newcommand\TDsTikzX[1]{$x_#1$}
\newcommand\TDsTikzVoid[1]{}
\newif\iftdssubsamplebool
\newif\iffillv
\newif\ifsparsev
\newif\ifnoisycolorsv
\newif\ifrandomcolorsv
\newif\ifdrawvec
\tikzset{
	shift to anchor/.code={
		\tikz@scan@one@point\pgfutil@firstofone(-\tikz@anchor)\relax
		\pgfkeysalso{shift={(-\pgf@x,-\pgf@y)}}
	},
	% Draws a vector (rectangle) of dimensions (width=#1,heigt=#2) and label #3 in the middle.
	vector/args/width/.store in=\W,
	vector/args/width=0.5,
	vector/args/height/.store in=\H,
	vector/args/height=2,
	vector/args/label/.store in=\L,
	vector/args/label=$x$,
	vector/args/fill/.is if=fillv,
	vector/args/fill=false,
	vector/args/fill color/.store in=\fillcol,
	vector/args/fill color=black,
	vector/args/sparse/.is if=sparsev,
	vector/args/sparse=false,
	vector/args/noisy colors/.is if=noisycolorsv,
	vector/args/noisy colors=false,
	vector/args/noise level min/.store in=\noiselevelmin,
	vector/args/noise level min=30, % btw 0 and 100 (mixing proportion with white)
	vector/args/noise level max/.store in=\noiselevelmax,
	vector/args/noise level max=100, % btw 0 and 100 (mixing proportion with white)
	vector/args/random colors/.store in=\randomcolorsv,
	vector/args/random colors=false,
	vector/args/random colors/.default=true,
	vector/args/random colors saturation/.store in=\randomsat,
	vector/args/random colors saturation=100,
	vector/args/first color/.store in=\binaryfirstcolor,
	vector/args/first color=blue,
	vector/args/second color/.store in=\binarysecondcolor,
	vector/args/second color=yellow,
	vector/args/nonzero values/.store in=\nnz,
	vector/args/nonzero values=1,
	vector/args/values/.store in=\nbvals,
	vector/args/values=1,
	vector/args/seed/.store in=\vecseed,
	vector/args/seed=42,
	vector/args/drawvec/.is if=drawvec,
	vector/args/drawvec=true,
	vector/.pic={
		\pgfqkeys{/tikz/vector/args}{#1}
		\pgfmathsetseed{\vecseed}
		\pgfmathsetmacro\bx{-0.5*\W}
		\pgfmathsetmacro\by{-0.5*\H}
		\pgfmathsetmacro\ex{-\bx}
		\pgfmathsetmacro\ey{-\by}
		\def\defcords{
			\coordinate (-west) at (\bx,0);
			\coordinate (-east) at (\ex,0);
			\coordinate (-north) at (0,\ey);
			\coordinate (-north west) at (\bx,\ey);
			\coordinate (-north east) at (\ex,\ey);
			\coordinate (-south) at (0,\by);
			\coordinate (-south west) at (\bx,\by);
			\coordinate (-south east) at (\ex,\by);
			\coordinate (-center) at (0,0);
		}
		\defcords{}
		\begin{scope}[shift to anchor]
			\defcords{}
			\pgfmathsetmacro\hval{\H/\nbvals}
			\ifsparsev
				\foreach \x in {1,...,\nnz} {
					\pgfmathrandom{1,\nbvals}
					\pgfmathsetmacro\deby{\by+(\pgfmathresult-1)*\hval}
					\pgfmathsetmacro\endy{\deby+\hval}
					\pickcolor{rescol}{\fillcol}{\noiselevelmin}{\noiselevelmax}{\randomsat}
					\path[fill=rescol] (\bx,\deby) rectangle (\ex,\endy);
				}
			\else
				\iffillv
					\foreach \x in {1,...,\nbvals} {
						\pgfmathsetmacro\deby{\by+(\x-1)*\hval}
						\pgfmathsetmacro\endy{\deby+\hval}
						\pickcolor{rescol}{\fillcol}{\noiselevelmin}{\noiselevelmax}{\randomsat}
						\path[fill=rescol] (\bx,\deby) rectangle (\ex,\endy);
					}
				\fi
			\fi
			\ifdrawvec
				\draw (\bx,\by) rectangle (\ex,\ey);
			\fi
			\node[anchor=center] at (0,0) {\L};
		\end{scope}
	}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                              Datasets                               %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newif\ifnoisycolorsds
\newif\ifrandomcolorsds
\newif\iffillds
\newif\ifsparseds
\newif\iflinkends
\newif\iffillmiddle

\newcommand\drawvectorpic[3]{\pic[anchor=south west,#3] at (\result,0) {vector={width=\TDsVecWidth,height=\TDsHeight,values=\nbvalsds,nonzero values=\nnzds,fill color=\fillcolds,random colors saturation=\randomsatds,noise level min=\noiselevelminds,noise level max=\noiselevelmaxds,label=\TDsLabels{#1},seed=\tmpseed,#2}};}
\newcommand\dealwithnoisyandrandom[3]{
	\ifrandomcolorsds
		\drawvectorpic{#1}{random colors,#3}{#2}
	\else
		\ifnoisycolorsds
			\drawvectorpic{#1}{noisy colors,#3}{#2}
		\else
			\drawvectorpic{#1}{#3}{#2}
		\fi
	\fi

}
\newcommand\dealwithbooleans[2]{
	\iffillds
		\dealwithnoisyandrandom{#1}{#2}{fill}
	\else
		\ifsparseds
			\dealwithnoisyandrandom{#1}{#2}{sparse}
		\else
			\drawvectorpic{#1}{}{#2}
		\fi
	\fi
}
\tikzset{
	% Dataset e.g. [x_1, … , x_n].
	dataset/args/width/.store in=\TDsVecWidth,
	dataset/args/width=0.5,
	dataset/args/height/.store in=\TDsHeight,
	dataset/args/height=2,
	dataset/args/space between vectors/.store in=\TDsSpaceBtwVecs,
	dataset/args/space between vectors=0,
	dataset/args/number at beginning/.store in=\TDsNbBeg,
	dataset/args/number at beginning=3,
	dataset/args/middle space/.store in=\TDsMidSpace,
	dataset/args/middle space=0.2,
	dataset/args/labels/.store in=\TDsLabels,
	dataset/args/labels=\TDsTikzX,
	dataset/args/last label/.store in=\TDsLastLabel,
	dataset/args/last label=n,
	dataset/args/subsample/.is if=tdssubsamplebool,
	dataset/args/subsample=false,
	dataset/args/fill/.is if=fillds,
	dataset/args/fill=false,
	dataset/args/fill color/.store in=\fillcolds,
	dataset/args/fill color=black,
	dataset/args/nonzero values/.store in=\nnzds,
	dataset/args/nonzero values=1,
	dataset/args/values/.store in=\nbvalsds,
	dataset/args/values=1,
	dataset/args/sparse/.is if=sparseds,
	dataset/args/sparse=false,
	dataset/args/linkends/.is if=linkends,
	dataset/args/linkends=true,
	dataset/args/fillmiddle/.is if=fillmiddle,
	dataset/args/fillmiddle=false,
	dataset/args/random colors/.is if=randomcolorsds,
	dataset/args/random colors=false,
	dataset/args/random colors saturation/.store in=\randomsatds,
	dataset/args/random colors saturation=80,
	dataset/args/noisy colors/.is if=noisycolorsds,
	dataset/args/noisy colors=false,
	dataset/args/noise level min/.store in=\noiselevelminds,
	dataset/args/noise level min=30, % btw 0 and 100 (mixing proportion with white)
	dataset/args/noise level max/.store in=\noiselevelmaxds,
	dataset/args/noise level max=100, % btw 0 and 100 (mixing proportion with white)
	dataset/args/seed/.store in=\TDsRdmSeed,
	dataset/args/seed=23,
	dataset/tmpvector/.style={},
	dataset/.pic={
		\pgfqkeys{/tikz/dataset/args}{#1}
		\pgfmathsetseed{\TDsRdmSeed}
		% Compute total height/width
		\pgfmathsetmacro\wtot{(\TDsNbBeg+2)*\TDsVecWidth+(\TDsNbBeg+1)*\TDsSpaceBtwVecs+\TDsMidSpace}
		\pgfmathsetmacro\htot{\TDsHeight}
		\pgfmathsetmacro\anchYmid{0.5*\htot}
		\pgfmathsetmacro\anchXmid{0.5*\wtot}
		% Position anchors
		\def\defcords{
			\coordinate (-west) at (0,\anchYmid);
			\coordinate (-east) at (\wtot,\anchYmid);
			\coordinate (-north) at (\anchXmid,\htot);
			\coordinate (-south) at (\anchXmid,0);
			\coordinate (-center) at (\anchXmid,\anchYmid);
			\coordinate (-north west) at (0,\htot);
			\coordinate (-north east) at (\wtot,\htot);
			\coordinate (-south west) at (0,0);
			\coordinate (-south east) at (\wtot,0);
		}
		\defcords{}
		\begin{scope}[shift to anchor]
			\pgfmathsetmacro\hzmidspacebegin{\TDsNbBeg*(\TDsVecWidth+\TDsSpaceBtwVecs)}
			\pgfmathsetmacro\hzmidspaceend{(\TDsNbBeg+1)*(\TDsVecWidth+\TDsSpaceBtwVecs)+\TDsMidSpace}
			% Middle space
			\iffillmiddle
				\fill[\fillcolds] (\hzmidspacebegin,0) rectangle (\hzmidspaceend,\TDsHeight);
			\fi
			\iflinkends
				\draw[dashed] (\hzmidspacebegin,\TDsHeight) -- (\hzmidspaceend,\TDsHeight);
				\draw[dashed] (\hzmidspacebegin,0) -- (\hzmidspaceend,0);
			\fi
			\foreach \x in {1,...,\TDsNbBeg} {
				\pgfmathsetmacro\tmpseed{\TDsRdmSeed+\x}
				\pgfmathsetmacro\result{(\x-1)*(\TDsVecWidth+\TDsSpaceBtwVecs)}
				\pgfmathsetmacro\endvec{\result+\TDsVecWidth}
				\iftdssubsamplebool
					\pgfmathrandom{2}
					\ifthenelse{\lengthtest{\pgfmathresult pt > 1pt}}{
						\pgfqkeys{/tikz/dataset/tmpvector}{.style={opacity=0.25}}
					}{
						\pgfqkeys{/tikz/dataset/tmpvector}{.style={opacity=1}}
					}
				\fi
				%\def\tmplabel{\TDsLabels{\x}}
				\dealwithbooleans{\x}{/tikz/dataset/tmpvector}
				\global\let\endvecmemorize=\endvec
			}
			\pgfmathsetmacro\tmpseed{\TDsRdmSeed+\TDsNbBeg+1}
			\pgfmathsetmacro\resx{(\TDsNbBeg+0.5)*(\TDsVecWidth+\TDsSpaceBtwVecs)+0.5*\TDsMidSpace}
			\pgfmathsetmacro\result{(\TDsNbBeg+1)*(\TDsVecWidth+\TDsSpaceBtwVecs)+\TDsMidSpace}
			%\pgfmathsetmacro\resultto{\result+\TDsVecWidth}
			\dealwithbooleans{\TDsLastLabel}{}
			\node[anchor=center] at (\resx,\anchYmid){$\cdots$};
			\defcords{}
		\end{scope}
	},
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                          Diagonal matrices                          %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\drawrectdiagmat[3]{\pic[anchor=north west,#3] at (\posbeg,\poscomp) {vector={width=\sizeoneblock,height=\sizeoneblock,fill color=\fillcolds,random colors saturation=\randomsatds,noise level min=\noiselevelminds,noise level max=\noiselevelmaxds,label=\DMsLabels{#1},seed=\tmpseed,drawvec=false, first color=\binaryfirstcolordiagmat, second color=\binarysecondcolordiagmat, #2}};}
\newcommand\dealwithnoisyandrandomdiagmat[3]{
	\ifthenelse{\equal{\randomcolorsdiagmat}{false}}{
		\ifnoisycolorsds
			\drawrectdiagmat{#1}{noisy colors,#3}{#2}
		\else
			\drawrectdiagmat{#1}{#3}{#2}
		\fi
	}{
		\drawrectdiagmat{#1}{random colors=\randomcolorsdiagmat,#3}{#2}
	}

}
\newcommand\dealwithbooleansdiagmat[2]{
	\iffillds
		\dealwithnoisyandrandomdiagmat{#1}{#2}{fill}
	\else
		\drawrectdiagmat{#1}{}{#2}
	\fi
}
\tikzset{
	% Dataset e.g. [x_1, … , x_n].
	diagmat/args/size/.store in=\DMsSize,
	diagmat/args/size=0.5,
	diagmat/args/dimension/.store in=\DMsDim,
	diagmat/args/dimension=10,
	diagmat/args/labels/.store in=\DMsLabels,
	diagmat/args/labels=\TDsTikzVoid,
	diagmat/args/last label/.store in=\DMsLastLabel,
	diagmat/args/last label=n,
	diagmat/args/fill/.is if=fillds,
	diagmat/args/fill=false,
	diagmat/args/fill color/.store in=\fillcolds,
	diagmat/args/fill color=black,
	diagmat/args/random colors/.store in=\randomcolorsdiagmat,
	diagmat/args/random colors=false,
	diagmat/args/random colors/.default=true,
	diagmat/args/random colors saturation/.store in=\randomsatds,
	diagmat/args/random colors saturation=80,
	diagmat/args/first color/.store in=\binaryfirstcolordiagmat,
	diagmat/args/first color=red,
	diagmat/args/second color/.store in=\binarysecondcolordiagmat,
	diagmat/args/second color=orange,
	diagmat/args/noisy colors/.is if=noisycolorsds,
	diagmat/args/noisy colors=false,
	diagmat/args/noise level min/.store in=\noiselevelminds,
	diagmat/args/noise level min=30, % btw 0 and 100 (mixing proportion with white)
	diagmat/args/noise level max/.store in=\noiselevelmaxds,
	diagmat/args/noise level max=100, % btw 0 and 100 (mixing proportion with white)
	diagmat/args/seed/.store in=\DMsRdmSeed,
	diagmat/args/seed=23,
	diagmat/.pic={
		\pgfqkeys{/tikz/diagmat/args}{#1}
		\pgfmathsetseed{\DMsRdmSeed}
		% Compute total height/width
		\pgfmathsetmacro\halfwidth{0.5*\DMsSize}
		% Position anchors
		\def\defcords{
			\coordinate (-west) at (0,\halfwidth);
			\coordinate (-east) at (\DMsSize,\halfwidth);
			\coordinate (-north) at (\halfwidth,\DMsSize);
			\coordinate (-south) at (\halfwidth,0);
			\coordinate (-center) at (\halfwidth,\halfwidth);
			\coordinate (-north west) at (0,\DMsSize);
			\coordinate (-north east) at (\DMsSize,\DMsSize);
			\coordinate (-south west) at (0,0);
			\coordinate (-south east) at (\DMsSize,0);
		}
		\defcords{}
		\begin{scope}[shift to anchor]
			\pgfmathsetmacro\sizeoneblock{\DMsSize/\DMsDim}
			\foreach \x in {1,...,\DMsDim} {
				\pgfmathsetmacro\tmpseed{\DMsRdmSeed+\x}
				\pgfmathsetmacro\posbeg{(\x-1)*\sizeoneblock}
				\pgfmathsetmacro\poscomp{\DMsSize-\posbeg}
				\dealwithbooleansdiagmat{}{}
			}
			\draw[] (0,0) rectangle (\DMsSize,\DMsSize);
			\defcords{}
		\end{scope}
	},
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                              Hadamard                               %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\drawhad[6]{
	\begingroup
	\pgfmathtruncatemacro\tmplevel{#1}
	\pgfmathtruncatemacro\tmppar{#2}
	\pgfmathsetmacro\tmpt{#3}
	\pgfmathsetmacro\tmpf{#4}
	\pgfmathsetmacro\tmpfv{#5}
	\pgfmathsetmacro\tmps{#6}
	\ifnum #1=1
		%\fill[gray] (#3,#4) rectangle (#5,#6);
		\ifnum #2=1
			\fill[\fgcolor] (#3,#4) rectangle (#5,#6);
		\else
			\fill[\bgcolor] (#3,#4) rectangle (#5,#6);
		\fi
	\else
		\pgfmathtruncatemacro\newlogdim{#1 - 1}
		\pgfmathtruncatemacro\newparity{1 - #2}
		\pgfmathsetmacro\midx{#3 + 0.5*(#5 - #3)}
		\pgfmathsetmacro\midy{#4 + 0.5*(#6 - #4)}
		\drawhad{\newlogdim}{\tmppar}{\tmpt}{\midy}{\midx}{\tmps} % top left
		\drawhad{\newlogdim}{\tmppar}{\midx}{\midy}{\tmpfv}{\tmps} % top right
		\drawhad{\newlogdim}{\tmppar}{\tmpt}{\tmpf}{\midx}{\midy} % bottom left
		\drawhad{\newlogdim}{\newparity}{\midx}{\tmpf}{\tmpfv}{\midy} % bottom right
	\fi
	\endgroup
}

\tikzset{
	hadamard/args/size/.store in=\HADSize,
	hadamard/args/size=0.5,
	hadamard/args/logdim/.store in=\HADLogDim,
	hadamard/args/logdim=4,
	hadamard/args/fill color/.store in=\fillcolds,
	hadamard/args/fill color=black,
	hadamard/args/fg color/.store in=\fgcolor,
	hadamard/args/fg color=black,
	hadamard/args/bg color/.store in=\bgcolor,
	hadamard/args/bg color=white,
	hadamard/.pic={
		\pgfqkeys{/tikz/hadamard/args}{#1}
		% Compute total height/width
		\pgfmathsetmacro\halfwidth{0.5*\HADSize}
		% Position anchors
		\def\defcords{
			\coordinate (-west) at (0,\halfwidth);
			\coordinate (-east) at (\HADSize,\halfwidth);
			\coordinate (-north) at (\halfwidth,\HADSize);
			\coordinate (-south) at (\halfwidth,0);
			\coordinate (-center) at (\halfwidth,\halfwidth);
			\coordinate (-north west) at (0,\HADSize);
			\coordinate (-north east) at (\HADSize,\HADSize);
			\coordinate (-south west) at (0,0);
			\coordinate (-south east) at (\HADSize,0);
		}
		\defcords{}
		\begin{scope}[shift to anchor]
			\drawhad{\HADLogDim}{1}{0}{0}{\HADSize}{\HADSize}
			\draw (0,0) rectangle (\HADSize,\HADSize);
			\defcords{}
		\end{scope}
	},
}

